Statistically Significant Stopping of Neural Network Training

The general approach taken when training deep learning classifiers is to save the parameters after every few iterations, train until either a human observer or a simple metric-based heuristic decides the network isn't learning anymore, and then backtrack and pick the saved parameters with the best validation accuracy. Simple methods are used to determine if a neural network isn't learning anymore because, as long as it's well after the optimal values are found, the condition doesn't impact the final accuracy of the model. However from a runtime perspective, this is of great significance to the many cases where numerous neural networks are trained simultaneously (e.g. hyper-parameter tuning). Motivated by this, we introduce a statistical significance test to determine if a neural network has stopped learning. This stopping criterion appears to represent a happy medium compared to other popular stopping criterions, achieving comparable accuracy to the criterions that achieve the highest final accuracies in 77% or fewer epochs, while the criterions which stop sooner do so with an appreciable loss to final accuracy. Additionally, we use this as the basis of a new learning rate scheduler, removing the need to manually choose learning rate schedules and acting as a quasi-line search, achieving superior or comparable empirical performance to existing methods.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> macros.tex <==
\newcommand{\R}{\mathbb{R}}
\newcommand{\Na}{\mathbb{N}}
\newcommand{\Zi}{\mathbb{Z}}
\newcommand{\gauss}[2]{\Gamma_{#1,#2}}
\newcommand{\bern}[1][p]{B_{#1}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\aN}{N}
\newcommand{\agentset}{[\aN]}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\todo}[1]{\textcolor{red}{#1}}
\newcommand{\transition}{P}
\newcommand{\reward}{R}
\newcommand{\observations}{\Omega}
\newcommand{\obsfunc}{O}
\newcommand{\observation}{\omega}
\DeclarePairedDelimiter{\set}{\{}{\}}
\newcommand{\pol}{\pi}
\newcommand{\modelname}{Multi-Agent Informational Learning Process}
\newcommand{\modelabbr}{MAILP}
\newcommand{\coord}{\mathcal{C}}
\newcommand{\kval}{\mathcal{K}}
\newcommand{\info}{\mathcal{I}}
\newcommand{\learnfunc}{\Lambda}
\newcommand{\funcdef}[3]{#1\colon {#2 \to #3 }}

\newcommand{\mc}[1]{\multicolumn{2}{c}{#1}}

==> xr-overleaf.tex <==
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
